On the Monniaux Problem in Abstract Interpretation

The Monniaux Problem in abstract interpretation asks, roughly speaking, whether the following question is decidable: given a program $P$, a safety (\emph{e.g.}, non-reachability) specification $\varphi$, and an abstract domain of invariants $\mathcal{D}$, does there exist an inductive invariant $I$ in $\mathcal{D}$ guaranteeing that program $P$ meets its specification $\varphi$. The Monniaux Problem is of course parameterised by the classes of programs and invariant domains that one considers. In this paper, we show that the Monniaux Problem is undecidable for unguarded affine programs and semilinear invariants (unions of polyhedra). Moreover, we show that decidability is recovered in the important special case of simple linear loops.

==> lower_more_one.tex <==
\subsection{Stuff on semilinear sets}
\todo[inline]{This will probably need to be included in the preliminary section eventually.}

\newcommand{\dotprod}[2]{\langle#1,#2\rangle}

I use the notation $\dotprod{x}{y}$ for the dot product in $\C$: $\dotprod{x}{y}=\Re{x\overline{y}}$
(also equals $x\odot y$ used in the rest of the document at the moment). A \emph{ray} of $\C^n$
is any set of the form $x+\Rp z=\set{x+tz:t\geqslant0}$ where $x,z\in\C^n$. A \emph{subray}
of a ray $R$ is any ray $R'\subseteq R$. A \emph{half-space} of $\C^n$ is any set of the form
$\set{z:\dotprod{z}{x}\geqslant\alpha}$ for some $x\in\C^n\setminus{0}$ and $\alpha\in\R$.
A \emph{quarter-space}

Recall that by the Minkowski-Weyl theorem, any convex polyhedron is the Minkowski sum of a polytope
and a finitely generated cone.

Recall that any matrix $A\in\C^{p\times n}$ is equivalent to $\pi_r$ where $r$ is the rank of $A$,
and $\pi_r$ is the matrix of the projection $(x_1,\ldots,x_n)\mapsto(x_1,\ldots,x_r,0,\ldots,0)$,
\emph{ie} there exists $P\in\C^{n\times n}$ and $Q\in\C^{p\times p}$ invertible such that $A=Q\pi_rP$.

\begin{lemma}\label{lem:semilin_unbounded_ray}
A semilinear set is unbounded if and only if it is contains a ray.
\end{lemma}
\begin{proof}
For a convex polyhedron, use the Minkowski-Weyl theorem. Then use the fact that a semilinear set
is a \emph{finite} union of convex polyhedra.
\end{proof}

\begin{lemma}\label{lem:semilin_affine_bounded_ray}
Let $\mathcal{I}\subseteq\C^n$ be a semilinear set and $f:\C^n\to\C^p$ be an affine function.
Then $f(\mathcal{I})$ is bounded if and only if $f(R)$ is bounded for every ray $R\subseteq\mathcal{I}$.
\end{lemma}
\begin{proof}
If $f(\mathcal{I})$ is bounded then in particular $f(L)\subseteq f(\mathcal{I})$ is bounded for every
ray $L\subseteq\mathcal{I}$. Conversely assume that $f(\mathcal{I})$ is unbounded. Since $\mathcal{I}$
is a finite union of convex polyhedra and affine maps preserve convexity and boundedness, it must be the case
that $f(\mathcal{P})$ is unbounded, for some convex polyhedron $\mathcal{P}\subseteq\mathcal{I}$.
Let $\mathcal{P}=P+C$ be the Minkowski-Weyl decomposition of $\mathcal{P}$, let $A\in\C^{p\times n}$
be the linear part of $f$. Then $f(\mathcal{P})=f(P)+AC$ but but $f(P)$ is bounded since $P$ is
a polytope, thus $AC$ must be unbounded. In particular, $C$ contains a ray $R$ such that $AR$ is unbounded.
It follows that $f(R)=f(0)+AC$ is unbounded.
\end{proof}

\begin{lemma}\label{lem:semilin_inverse_proj_ray}
Let $\mathcal{I}\subseteq\C^n$ be a semilinear set and $f:\C^n\to\C^r$ an affine map.
Assume that $f(\mathcal{I})$ contains a ray $R$, then there exists a ray $R'\subseteq\mathcal{I}$
such that $f(R')$ is a subray of $R$.
More precisely, if $R=x_0+\Rp u$ then there exists $\alpha\geqslant0$ and $y_0,v\in\C^n$
such that for all $t\geqslant\alpha$, $y_0+tv\in\mathcal{I}$ and $f(y_0+tv)=x_0+tu$,
in particular $R'=y_0+\R_{\geqslant\alpha}v$.
\end{lemma}
\begin{proof}
First note that the second part of the lemma follows from the first. Indeed, if $f(R')$ is a subray
of $R$, then $f(R')=x_0+\R_{\geqslant\alpha}u$ for some $\alpha$. Let $y_1,y_2\in R'$ such that
$f(y_1)=x_0+\alpha u$ and $f(y_2)=x_0+(1+\alpha)u$. Define $v=y_2-y_1$ and $y_0=y_1-\alpha v$,
then
\[f(y_0)=f(y_1)-\alpha(f(y_2)-f(y_1))=(1+\alpha)f(y_1)-\alpha f(y_2)=x_0\]
and
\[f(y_0+tv)=f(y_0)+t(f(y_2)-f(y_1))=x_0+t(f(y_2)-f(y_1))=x_0+tu.\]
Finally since $y_1,y_2\in R'$, it is not hard to see that $y_0+tv\in R'$ for all $t\geqslant\alpha$.


To prove the lemma, write $R=x_0+\Rp u$ and let $\mathcal{S}=\set{(z,t)\in\mathcal{I}\times\Rp:f(z)=x_0+tu}$
which is semilinear. Let $\pi_1:\C^{n+1}\to\C,(z,t)\mapsto z$ and $\pi_2:\C^{n+1}\to\C,(z,t)\mapsto t$ which are affine.
Observe that by hypothesis, for all $t\geqslant0$, $x_0+tu\in R$ and
$R\subseteq f(\mathcal{I})$ thus there exists $z\in\mathcal{I}$ such that $f(z)=x_0+tu$.
Hence $\pi_2(\mathcal{S})=\Rp$ is unbounded and by Lemma~\ref{lem:semilin_affine_bounded_ray},
there exists a ray $R'\subseteq\mathcal{S}$ such that $\pi_2(R')$ is unbounded. But since $\pi$
is affine, $R'$ is a ray and $\pi_2(R')\subseteq\Rp$, $\pi_2(R')$ must be a ray, \emph{ie} $\pi_2(R')=\R_{\geqslant\alpha}$
for some $\alpha\geqslant0$. Let $R''=\pi_1(R')\subseteq\mathcal{I}$ which is also a ray, we claim
that $f(R'')=x_0+\R_{\geqslant\alpha}u$, which concludes since it is a subray of $R$.
Indeed, for all $t\geqslant\alpha$, there exists $z\in\pi_1(R')$ such that $(z,t)\in R'$.
But then $(z,t)\in\mathcal{S}$, so $f(z)=x_0+tu$. Thus $f(R'')\supseteq x_0+\R_{\geqslant\alpha}u$,
the other inclusion is trivial.
\end{proof}

\begin{corollary}\label{cor:semilinear_unproj_ray}
Let $\mathcal{I}\subseteq\C^{n+m}$ semilinear and assume that
$\set{y\in\C^m:\exists x\in\C^n,(x,y)\in\mathcal{I}}$ contains a ray $y_0+\Rp v$. Then there exists $x_0,u\in\C^n$
and $\alpha\geqslant0$ such that for all $t\geqslant\alpha$, $(x_0+tu,y_0+tv)\in\mathcal{I}$.
\end{corollary}

\begin{lemma}\label{cor:semilin_inverse_proj_hspace}
Let $\mathcal{I}\subseteq\C^2$ semilinear, let $\pi_i:\C^2\to\C,x\mapsto x_i$ and assume that
$\pi_2(\mathcal{I})$ contains a half-space $\mathcal{H}=\set{z\in\C:\dotprod{z}{\tau}\geqslant\alpha}$.
Then there exists $\beta\geqslant\alpha$, $\gamma\in\R$, $\sigma\in\set{1,2}$, $x,u,v\in\C$
such that for all $t\geqslant\beta$ and $s\geqslant\gamma$,
\[(x+tu+sv,t\tau+si^\sigma\tau)\in\mathcal{I}.\]
\end{lemma}

\subsubsection{Root of unity}

\begin{lemma}
\label{lem:lower_more_one_diag_one_rou}
Let $\lambda=\rho e^{i\theta}$ with $\rho>1$ and $\theta=\tfrac{2p}{q}\pi$, and $x$ be a non-zero complex number.
For any $\alpha\geqslant0$, define
\[\mathcal{I}_{\alpha}=\bigcup_{k=0}^{q-1}\mathcal{I}_{\alpha,k}
    \qquad\text{where}\qquad
    \mathcal{I}_{\alpha,k}=\R_{\geqslant\alpha}\lambda^kx.\]
Let $\I\subseteq\C$ be a non-empty closed semilinear set stable under $\lambda$ and containing $x$, then
there exists $\alpha\geqslant0$ such that $\mathcal{I}_\alpha\subseteq\mathcal{I}$. Furthermore,
$\mathcal{I}_\alpha$ is stable under $\lambda$ and contains $x$.
\end{lemma}

\begin{proof}
Let $\mathcal{J}=\mathcal{I}\cap\Rp x$, note that this is a semilinear set of (real) dimension $1$.
Observe that all the points $x_{k}=\lambda^{qk}x$ belong to $\mathcal{J}$ since $\lambda^q\in\Rp$.
Furthermore, $|x_k|=\rho^k|x|$ tends to infinity as $k$ increases since $\rho>1$.
It follows that $\mathcal{J}$ is infinite and unbounded, hence it must contain an infinite interval,
that is there exists $\alpha\geqslant0$ such that
$\R_{\geqslant\alpha}x=\mathcal{I}_{\alpha,0}\subseteq\mathcal{J}$.
But since $\mathcal{I}$ is stable under $\lambda$, it must be the case that
$\lambda^k\mathcal{I}_{\alpha,0}=\mathcal{I}_{\alpha,k}\subseteq\mathcal{I}$
which concludes the first part of the lemma. Finally, observe that
$\lambda\mathcal{I}_{\alpha,q-1}=\rho^q\mathcal{I}_{\alpha,0}\subseteq\mathcal{I}_{\alpha,0}$
thus $\mathcal{I}_\alpha$ is stable under $\lambda$.
\end{proof}

\subsection{Dimension 1}

\subsubsection{Not a root of unity}

\begin{lemma}
\label{lem:lower_more_one_diag_one_nrou}
Let $\lambda=\rho e^{i\theta}$ with $\rho>1$ and $\theta$ an irrational multiple of $\pi$,
and $x$ be a non-zero complex number.
For any $\alpha\geqslant0$, define
\[\mathcal{I}_{\alpha}=\]
Let $\I\subseteq\C$ be a non-empty closed semilinear set stable under $\lambda$ and containing $x$, then
there exists $\alpha\geqslant0$ such that $\mathcal{I}_\alpha\subseteq\mathcal{I}$. Furthermore,
$\mathcal{I}_\alpha$ is stable under $\lambda$ and contains $x$.
\end{lemma}

\begin{proof}
For any $\alpha,\phi\in\R$, define $\mathcal{I}_{\phi,\alpha}=\R_{\geqslant\alpha}e^{i\phi}x$ which
is semilinear.
Let $\phi\in[0,2\pi)$, then
$\mathcal{I}_{\phi,0}\cap\mathcal{I}$ is a semilinear set of (real) dimension $1$, that is a
finite union of intervals and points. If it contains an infinite interval then by taking $\alpha$ big
enough we can ensure that $\mathcal{I}_{\phi,\alpha}\subseteq\mathcal{I}$. Otherwise it must be bounded,
and we can find
$\alpha\in\Rp$ such that $\mathcal{I}_{\phi,\alpha}\cap\mathcal{I}=\varnothing$. Assume
the latter case. Then we must have $\lambda^{-1}\mathcal{I}_{\phi,\alpha}\cap\mathcal{I}=\varnothing$, since $\mathcal{I}$
is stable under $\lambda$. Since $\rho>1$, we have
$\lambda^{-1}\mathcal{I}_{\phi,\alpha}=\mathcal{I}_{\phi-\theta,\alpha\rho^{-1}}\supseteq\mathcal{I}_{\phi-\theta,\alpha}$
and thus $\mathcal{I}_{\phi-\theta,\alpha}\cap\mathcal{I}=\varnothing$.
Applying this argument repeatedly we get that $C\cap\mathcal{I}=\varnothing$ where $C=\bigcup_{n\in\N}\mathcal{I}_{\phi-n\theta,\alpha}$.
Let $B=\set{zx:z\in\C\text{ and }\infnorm{z}=\alpha}$ be a (transformed) box of size $2\alpha$ around $0$. Note that $B$
is a semilinear set and that $B\cap \mathcal{I}_{\phi-n\theta,\alpha}$ is a single point
for all $n$. Furthermore, the set $\set{\phi-n\theta\mod 2\pi:n\in\N}$ is dense in $[0,2\pi)$ since
$\theta$ is an irrational multiple of $\pi$. Therefore $C\cap B$ is dense in $B$.
Let $X=\set{z\in B:\R_{\geqslant 1}z\cap\mathcal{I}=\varnothing}$, it is semilinear and
$C\cap B\subseteq X$. Indeed if $z\in C\cap B$ then $z=\beta e^{i(\phi-n\theta)}z$ for some $\beta\geqslant\alpha$
and $n\in\N$, and $\mathcal{I}_{\phi-n\theta,\alpha}\cap\mathcal{I}=\varnothing$. But then
$\R_{\geqslant 1}z\subseteq \mathcal{I}_{\phi-n\theta,\alpha}$ thus $z\in X$. As a consequence,
$\closure{X}=B$. Similarly, define $Y=\set{z\in B:\R_{\geqslant 1}z\cap\mathcal{I}\neq\varnothing}$:
it is semilinear and $X\cap Y=\varnothing$. Let $n_0\in\N$ be such that $\infnorm{\lambda^{n_0}x}\geqslant\alpha\infnorm{x}$,
then for all $n\geqslant n_0$, there exists $z_n\in B$ such that $\lambda^nx\in\R_{\geqslant 1}z_n$,
thus $z_n\in Y$. Let $Z=\set{z_n:n\in\N}$, note that $z_n=\beta_n\lambda^nx=\beta_n\rho^n e^{in\theta}x$
and again $\set{n\theta\mod 2\pi}$ is dense in $[0,2\pi)$, thus $Z$ is dense in $B$. But $Z$ is a
subset of $Y$ so $\closure{Y}=B$. We have reached a contradiction since $X,Y$ are semilinear, disjoint
and $\closure{X}=\closure{Y}=B$.

\textcolor{red}{rephrase everything above using new $\mathcal{I}_{z,\alpha}$ below?}\\
The above shows that for every $\phi\in[0,2\pi)$, there exists $\alpha\in\Rp$ such that
$\mathcal{I}_{\phi,\alpha}\subseteq\mathcal{I}$. We rephrase it as follows: let $B=\set{z\in\C:\infnorm{z}=1}$
be a box, it is semilinear. For every $z\in B$, let $\mathcal{I}_{z,\alpha}=\R_{\geqslant 1}zx$.
Then for every $z\in B$, there exists $\alpha\in\Rp$ such that $\mathcal{I}_{z,\alpha}\subseteq \mathcal{I}$.
We can define $f:B\to\Rp$ by $f(z)=\inf{\alpha\in\Rp:\mathcal{I}_{z,\alpha}\subseteq \mathcal{I}}$,
which is well-defined. This function has a semilinear graph and we claim that therefore it is
piecewise linear. In particular, it is bounded since $B$ is compact. It follows that there exists
$\alpha\in\Rp$ such that for all $z\in B$, $\mathcal{I}_{z,\alpha}\subseteq \mathcal{I}$.

FINISH this: from there we get that $\mathcal{I}$ essentially contains everything at infinity. In 
other words, $\mathcal{I}$ is made up of a bounded semilinear set + the complement of a bounded polyhedron.

% Recall that $Cx\cap\mathcal{I}=\varnothing$, thus $B x\cap\mathcal{I}$ is semilinear and its complement
% in $B x$ is dense. We conclude (probably a general fact for o-minimal sets?) that $B x\cap\mathcal{I}$
% is finite. Furthermore, its cardinal does not depend on $\alpha$
% 
% 
% Let $\mathcal{J}=\mathcal{I}\cap\Rp x$, note that this is a semilinear set of (real) dimension $1$.
% Observe that all the points $x_{k}=\lambda^{qk}x$ belong to $\mathcal{J}$ since $\lambda^q\in\Rp$.
% Furthermore, $|x_k|=\rho^k|x|$ tends to infinity as $k$ increases since $\rho>1$.
% It follows that $\mathcal{J}$ is infinite and unbounded, hence it must contain an infinite interval,
% that is there exists $\alpha\geqslant0$ such that
% $\R_{\geqslant\alpha}x=\mathcal{I}_{\alpha,0}\subseteq\mathcal{J}$.
% But since $\mathcal{I}$ is stable under $\lambda$, it must be the case that
% $\lambda^k\mathcal{I}_{\alpha,0}=\mathcal{I}_{\alpha,k}\subseteq\mathcal{I}$
% which concludes the first part of the lemma. Finally, observe that
% $\lambda\mathcal{I}_{\alpha,q-1}=\rho^q\mathcal{I}_{\alpha,0}\subseteq\mathcal{I}_{\alpha,0}$
% thus $\mathcal{I}_\alpha$ is stable under $\lambda$.
\end{proof}

